Modular Synthesis of Divide-and-Conquer Parallelism for Nested Loops (Extended Version)

We propose a methodology for automatic generation of divide-and-conquer parallel implementations of sequential nested loops. We focus on a class of loops that traverse read-only multidimensional collections (lists or arrays) and compute a function over these collections. Our approach is modular, in that, the inner loop nest is abstracted away to produce a simpler loop nest for parallelization. Then, the summarized version of the loop nest is parallelized. The main challenge addressed by this paper is that to perform the code transformations necessary in each step, the loop nest may have to be augmented (automatically) with extra computation to make possible the abstraction and/or the parallelization tasks. We present theoretical results to justify the correctness of our modular approach, and algorithmic solutions for automation. Experimental results demonstrate that our approach can parallelize highly non-trivial loop nests efficiently.

==> proofs/tcomp.tex <==
\begin{proposition}\label{prop:app:tcomp}
For a rightward function $f: \seq^n \to D$ with time complexity $O(m^n)$ defined through the recursive equation $f(\sigma \ccat [\delta]) =  f(\sigma) \otimes \mathbbm{G}(f(\sigma, d))(\delta)$
we have:
\begin{itemize}
\item Every $g \in \mathbbm{G}$ is a  (leftward or) rightward function of complexity $O(m^{n-1})$.
\item Any $d \in D$ is strictly of space complexity $O(m^{n-1})$\footnote{This is under the assumption that the data is fully read. So, this excludes, for example, operations on lists performed through reference manipulation without reading the entire list content.}.
\item $\otimes$ is computable in time $O(m^{n-1})$.
\end{itemize}
\end{proposition}
The proof of this proposition is straightforward, in that, if any of the upper bounds are violated, then one can show that the time complexity of $f$ would surpass $O(m^n)$.

Now, if $h_L$ is a homomorphism and we want the parallel computation based on the homomorphism's {\em join} operator $\odot$ to have the same complexity as $h_L$, we can use Proposition \ref{prop:app:tcomp} in place of \ref{prop:tcomp}. $\odot$ replaces $\otimes$, and we can conclude $\odot \in O(m^{n-1})$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

